Probabilistic Categorical Adversarial Attack & Adversarial Training

The existence of adversarial examples brings huge concern for people to apply Deep Neural Networks (DNNs) in safety-critical tasks. However, how to generate adversarial examples with categorical data is an important problem but lack of extensive exploration. Previously established methods leverage greedy search method, which can be very time-consuming to conduct successful attack. This also limits the development of adversarial training and potential defenses for categorical data. To tackle this problem, we propose Probabilistic Categorical Adversarial Attack (PCAA), which transfers the discrete optimization problem to a continuous problem that can be solved efficiently by Projected Gradient Descent. In our paper, we theoretically analyze its optimality and time complexity to demonstrate its significant advantage over current greedy based attacks. Moreover, based on our attack, we propose an efficient adversarial training framework. Through a comprehensive empirical study, we justify the effectiveness of our proposed attack and defense algorithms.

==> unused.tex <==
\begin{figure*}[h!]
    \centering
    % \subfigure{
    %     \includegraphics[width=0.23\textwidth]{figure/tradeoff1.png}
    %     \label{label_for_cross_ref_1}
    % }
 %    \subfigure{
	% \includegraphics[width=0.23\textwidth]{figure/tradeoff2.png}
 %        \label{label_for_cross_ref_2}
 %    }
 %    % \quad  
    \begin{subfigure}{.4\textwidth}
    \includegraphics[width=0.35\textwidth]{figure/tradeoff3.png}
        \label{label_for_cross_ref_3}
        \caption{AG's News with budget 3}
    \end{subfigure}
    \begin{subfigure}{.4\textwidth}
\includegraphics[width=0.35\textwidth]{figure/tradeoff4.png}
     %\caption{AG's News with budget 4}
        \label{label_for_cross_ref_4}
        % \caption{AG's News with budget 4}
    }
    \caption{An illustration of trade-offs. The blue bar represents the accuracy($1-SR$) under different attacks} while the yellow bar represents the average running time. For both metrics, smaller indicates better performance. We show the results of 2 datasets with different budgets as illustrating examples. Existing methods all have high levels on at least one metric which makes them infeasible under some circumstances, while PCAA can keep both under low levels.
    \label{tradeoff.fig}
\end{figure*}

